Analyzing Incentives for Protocol Compliance in Complex Domains: A Case Study of Introduction-Based Routing

Formal analyses of incentives for compliance with network protocols often appeal to game-theoretic models and concepts. Applications of game-theoretic analysis to network security have generally been limited to highly stylized models, where simplified environments enable tractable study of key strategic variables. We propose a simulation-based approach to game-theoretic analysis of protocol compliance, for scenarios with large populations of agents and large policy spaces. We define a general procedure for systematically exploring a structured policy space, directed expressly to resolve the qualitative classification of equilibrium behavior as compliant or non-compliant. The techniques are illustrated and exercised through an extensive case study analyzing compliance incentives for introduction-based routing. We find that the benefits of complying with the protocol are particularly strong for nodes subject to attack, and the overall compliance level achieved in equilibrium, while not universal, is sufficient to support the desired security goals of the protocol.

==> arxiv ibrcomp/inner.tex <==
\begin{algorithm}
\caption{EGTA Inner Loop}
\label{alg:inner-loop}
\begin{algorithmic}
\Require Strategy space $\stratcand=(\stratcand_1,\dotsc,\stratcand_R)$, Empirical game $G(\stratcand)$, Regret threshold $\rthresh$, Numbers of required samples \( \minsamp \) and \( \mincsamp \)
%, verified Nash set $V_N$ = \{Nash profiles $p_v^1$ $p_v^2$...which outerloop failed to find beneficial strategy on them\}
\Ensure Confirmed mixed RSNE \( \{q: \epsilon(q) \le \rthresh \mathrm{; all\ deviations\ of\ } q \mathrm{\ evaluated}\}  \)

\State
\State $\mathit{foundConfirmed} \gets \mathbf{false}$ 
\While{ $\neg\mathit{foundConfirmed}$} 
	\Repeat
		\State $(\solcand_C,\solcand_U,\solcand_R) \gets$ $\mathit{GameAnalysis}(G(\stratcand), \rthresh)$
	\For{$q \in \solcand_U$}
		\State $\mathit{ScheduleDeviation}(\Support(q), \stratcand\setminus \mathit{StrategiesIn}(q),\minsamp)$
	\EndFor
	\Until{$\solcand_U$ is empty}
	\State	
	\If{$\solcand_C \neq \emptyset$}
		\State $\mathit{foundConfirmed} \gets \mathbf{true}$
		\For {$q \in \solcand_C$}
%			$G(S_q) \gets G(support(q))$
			\If {$\mathit{foundConfirmed}\wedge \mathit{minSamples}(\Support(q)) < \mincsamp$}
%				\State Schedule more samples for the support set of $q$
				\State $\mathit{ScheduleSubgame}(\mathit{StrategiesIn}, \mincsamp)$ 
				\State $\mathit{foundConfirmed} \gets \mathbf{false}$
 			\EndIf
		\EndFor

    \Else
        \State \( \mathit{explored}\gets \mathbf{false} \) 
 	    \For {$q \in \solcand_R$} 
	       \If {\( \neg\mathit{explored}\wedge \neg\mathit{Subgame}(\mathit{StrategiesIn}(q) + \mathit{BestResponse}(q)) \)}  
	           \State \( \mathit{explored}\gets \mathbf{true} \)
	           \State $\mathit{ScheduleSubgame}(\mathit{StrategiesIn}(q) + \mathit{BestResponse}(q), \mincsamp)$
           \EndIf
	     \EndFor
     \If {\( \neg\mathit{explored} \)}        
		\State $\mathit{ScheduleSubgame}(\mathit{incrSubgame}(), \minsamp)$
	\EndIf  
	\EndIf
\EndWhile 
\State \Return \( \solcand_C \)
\end{algorithmic}
\end{algorithm} 

Notes to Algorithm~\ref{alg:inner-loop}:  
\begin{enumerate}
	\item $\Support(q)$ denotes the support of a profile $q$.
	\item $\mathit{ScheduleDeviation}(Q, \mathcal{S},n)$ generates simulations for profiles formed by deviating from profiles in set \( Q \) to strategies in role:strategy mapping \( \mathcal{S} \), until at least \( n \) of each are accumulated.     
	\item $\mathit{ScheduleSubgame}(\mathcal{S}, n)$ generates simulations for profiles comprising strategies in role:strategy mapping \( \mathcal{S} \), until at least \( n \) of each are accumulated.     
\item $\mathit{incrSubgame}()$ returns a minimal strategy set that is not a complete subgame in the current empirical game.       
\item At termination, the empirical game over \( \stratcand \) is augmented such that all RSNE candidates are confirmed or refuted.
\end{enumerate}


==> arxiv ibrcomp/outer.tex <==
\begin{algorithm}
\caption{Strategy Exploration Outer Loop (non-compliant mode, role~\( \rho \))}
\label{alg:outer-loop}
\begin{algorithmic}
\Require Empirical game $G(\stratcand)$, 
Open confirmed solution candidates \( \solcand_C \), 
Numbers of required samples \( \minsamp \) and \( \mincsamp \),
Numbers of strategies to select \( m \) and \( m' \)
\Ensure New compliant strategy to add to $\stratcand_\rho$
\State
\State $q \gets \arg\max_{q\in \solcand_C}\compliance(q)$    
\State \( \mathit{SeedStrategies}\gets \Support(q_\rho) \)  
\State \( \mathit{Explored}\gets \stratcand_\rho \)  
\State \( \mathit{newPayoff}\gets -\infty \)  
                                                          
\Repeat
  \State \( \mathit{bestPayoff}\gets \mathit{newPayoff} \)  
  \State \( \mathit{CandSet}\gets \LocalSearch(\mathit{SeedStrategies},\mathit{Explored},\mathbf{non\-compliant}) \)
  \State $\mathit{ScheduleDeviation}(\Support(q), \mathit{CandSet},\minsamp)$
  \State \( \mathit{Explored}\gets \mathit{Explored}\cup\mathit{CandSet} \) 
  \State $\mathit{ScheduleDeviation}(\Support(q), \mathit{SelectBestDeviators}(q,\rho,\mathit{CandSet},m), \mincsamp)$
  \State  \( \mathit{SeedStrategies}\gets \mathit{SelectBestDeviators}(q,\rho,\mathit{CandSet},m') \)
  \State \( \mathit{newPayoff}\gets \max_{s\in\mathit{SeedStrategies}}(u_\rho(s,q)) \)
\Until {\( \mathit{newPayoff} \le \mathit{bestPayoff} \)}
\State \Return \( \mathit{SelectBestDeviators}(q, \rho, \mathit{Explored}\setminus\stratcand_\rho, 1) \)		
\end{algorithmic} 
\end{algorithm}

Notes to Algorithm~\ref{alg:outer-loop}:
\begin{enumerate}  
	\item \( \LocalSearch(S_1,S_2,c) \) returns a nonempty set of strategy variations close to some strategy in \( S_1 \), distinct from \( S_2 \), and consistent with compliance state \( c \).
	\item \( u_\rho(s,q) \) denotes the payoff to a player of role \( \rho \) playing strategy \( s \) when the remaining players play according to profile \( q \).
	\item \( \mathit{SelectBestDeviators}(q,\rho,CS,m) \) evaluates the payoff to a role~\( \rho \) player deviating from profile \( q \) by playing \( s \), for each strategy \( s\in CS \). 
	It then returns the \( m \) best strategies according to this evaluation, or the entire set \( CS \) if \( \abs{CS}\le m \).
\end{enumerate}

